Pedagogy of Teaching Pointers in the C Programming Language using Graph Transformations

Visual learners think in pictures rather than words and learn best when they utilize representations based on graphs, tables, charts, maps, colors and diagrams. We propose a new pedagogy for teaching pointers in the C programming language using graph transformation systems to visually simulate pointer manipulation. In an Introduction to C course, the topic of pointers is often the most difficult one for students to understand; therefore, we experiment with graph-based representations of dynamic pointer structures to reinforce the learning. Groove, a graph transformation tool, is used to illustrate the behaviour of pointers through modelling and simulation. A study is presented to evaluate the effectiveness of the approach. This paper will also provide a comparison to other teaching methods in this area.

==> eptcsdata.tex <==
\providecommand{\firstpage}{117}
\providecommand{\publicationstatus}{J. Endrullis, D. Grzelak, T. Heindel and J. Kosiol (Eds):\\ GCM 2023 and GCM 2024\\
EPTCS 417, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.417.7}{10.4204/EPTCS.417.7}}
\pdfoutput=1

